Oops! Predicting Unintentional Action in Video

From just a short glance at a video, we can often tell whether a person's action is intentional or not. Can we train a model to recognize this? We introduce a dataset of in-the-wild videos of unintentional action, as well as a suite of tasks for recognizing, localizing, and anticipating its onset. We train a supervised neural network as a baseline and analyze its performance compared to human consistency on the tasks. We also investigate self-supervised representations that leverage natural signals in our dataset, and show the effectiveness of an approach that uses the intrinsic speed of video to perform competitively with highly-supervised pretraining. However, a significant gap between machine and human performance remains. The project website is available at https://oops.cs.columbia.edu

==> experiments.tex <==
\section{Experiments}\label{sec:exp}

The goal of our experiments is to analyze mid-level perceptual clues for recognizing intentionality in realistic video. To do this, we quantitatively evaluate the self-supervised methods on three tasks on our dataset (classification, localization, and anticipation). We also show quantitative ablations and qualitative visualizations to analyze limitations.

\begin{table}[tb]
\resizebox{\columnwidth}{!}{
\begin{center}
\begin{tabular}{l|c c | c}
\toprule
& \multicolumn{2}{c|}{\textbf{Linear Classifier}} & \textbf{Fine-tune} \\
\textbf{Method} & \textbf{All Labels} & \textbf{10\% Labels} & \textbf{All Labels}\\ \midrule
%Human Consistency & 72.4 & - & 72.4 \\
Kinetics Supervision  & 53.6 & 52.0 & 64.0                  \\ \midrule
Video Speed (ours)  & \textbf{53.4}  & \textbf{49.9}  & \textbf{61.6}             \\
Video Context \cite{oord2018representation}  & 50.0 & 47.2 & 60.3          \\
Video Sorting  \cite{xu2019self}    &     49.8 & 46.5 & 60.2         \\\midrule
Scratch    & 48.2 & 46.2 & 59.4              \\ 
Motion Magnitude     & 44.0 & -  & 44.0             \\
%Actions withheld  & 58.4            & -           \\ 
%Random withheld  & 58.4            & -           \\ \midrule
Chance & 33.3  &  33.3 & 33.3  \\ \bottomrule
\end{tabular}
\end{center}
}
\caption{\textbf{Classification Accuracy:} We evaluate performance of each self-supervised model versus baselines. We also compare against a model trained with Kinetics supervision to understand the gap between supervision and self-supervision. This results suggests learning to predict video speed is a promising form of video self-supervision.\vspace{-1em}}
\label{tab:cls}
\end{table}

\subsection{Baselines}

Besides the self-supervised methods above, we additionally compare against several other baselines. 

\textbf{Motion Magnitude:} We use simple motion detection as a baseline. To form this baseline, we compute optical flow \cite{ilg2017flownet} over the videos, and quantify the motion magnitude into a histogram. We experimented with several different bin sizes, and found that 100 bins performed the best. We then fit a multi-layer perceptron on the histogram, which is trained on the labeled portion of our training set to predict the three categories.

\begin{figure}[b]
\includegraphics[width=\columnwidth]{figs/closestvsmedian_filmstrip.pdf}
\vspace{-2em}
\caption{\textbf{Multi-modal Evaluation:} Unintentional actions cascade. For example, in this video, the person ``fails'' twice. To handle this in evaluation, we consider a prediction correct if it is sufficiently near any ground-truth label.}
\label{fig:closest} 
\end{figure}

\textbf{Kinetics Supervision:} We compare against a model that is trained on the full, annotated Kinetics action recognition dataset, which is either fine-tuned with our labeled training set, or used as a feature extractor. Since the model is trained on a large, labeled dataset of over $600,000$ videos, we do not expect our self-supervised models to outperform it. Instead, we use this baseline to understand the gap between supervised and self-supervised methods. 

\textbf{Linear versus Fine-tune:} Unless otherwise noted, the classifier is a linear classifier on the features from the last convolutional layer of the network. However, we also evaluated some models by fine-tuning, which we do to understand the best performance that one could obtain at this task. To fine-tune, we simply use the method as the network initialization, change the last layer to be the three-way classification task, and train the network end-to-end with stochastic gradient descent on our labeled set of videos.

\textbf{Fixed Priors:} We also compare against naive priors. We calculate the mode on the training set, and use this mode as the prediction. Additionally, we use chance. 

\textbf{Human Agreement:} To establish an upper expectation of performance on this dataset, we use a fourth, held-out worker's labels to measure human performance.

\subsection{Classification}\label{sec:exp_clsloc}

We first evaluate each model on a classification task. Given a short video clip, the task is to categorize it into one of the three categories (intentional, unintentional, or transitional). We extract one-second temporal windows in increments of $0.25$ seconds from the testing set.

Table \ref{tab:cls} reports classification accuracy for each method. All of the self-supervised methods outperform baselines, suggesting there are perceptual clues in unlabeled video for intentionality. The model trained with full Kinetics supervision obtains the best performance overall, indicating there is still no substitute for labeled data. However, the gap between the self-supervised models and supervised models is relatively small. For example, the best performing perceptual clue (video speed) is tied with Kinetics when large amounts of labels are available for training a linear layer. We also experimented with the reducing the number of examples in our labeled training set. While accuracy is positively correlated with number of labels, reducing the number of labels by an order of magnitude only causes a minor drop in performance.

\subsection{Localization}

We next evaluate temporal localization, which is challenging because it requires the model to detect the temporal boundary between intentional and unintentional action. We use our classifier in a sliding window fashion over the temporal axis, and evaluate whether the model can detect the point in time that the action switches from intentional to unintentional. The predicted boundary is the one with the most confident score of transition across all sliding windows.  Since videos can contain multiple transitional points, we consider the prediction correct if it sufficiently overlaps any of the ground truth positions in the dataset (Figure \ref{fig:closest}). We use two different thresholds of sufficient overlap: within one second, and within one quarter second.

Table \ref{tab:loc} reports accuracy at localizing the transition point. For both thresholds, the best performing self-supervised method is video speed, outperforming other self-supervised methods by over 10\%, which suggests that our video speed task learns more fine-grained video features.  Human consistency at this task is high ($88\%$ agreement), however there is still a large gap to both supervised and self-supervised approaches, underscoring the challenge of learning human intent in video. Figure \ref{fig:loc_results} shows a few qualitative results of localization as well as high-scoring false positives. The false positives suggest that our model commonly misses detecting unintentional action that requires knowledge, such as that cars usually do not drive on sidewalks. 


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/allresultsgrid.pdf}
\vspace{-2em}
\caption{\textbf{Example Localizations:} We show example predictions for localizing the transition to unintentional action. \textcolor[rgb]{0,.56,.12}{Green} indicates a correct prediction (within 0.25 sec). \textcolor[rgb]{.81,0,0}{Red} indicates a false alarm. \textcolor[rgb]{.81,.70,0}{Yellow} indicates a missed detection.\vspace{-1em}}
\label{fig:loc_results} 
\end{figure}



\begin{table}[tb]
\centering
% %\resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}l|cc|cc@{}}
% \toprule
%                 & \multicolumn{2}{c|}{\textbf{Error}} & \multicolumn{2}{c}{\textbf{Accuracy}} \\
% \textbf{Method} & \textbf{Normalized (\%)} & \textbf{Absolute (sec)} & \textbf{Within 1sec} & \textbf{Within 0.25s} \\ \midrule
% Human Consistency   & 6.4                    & 0.59                   & 88.0   & 62.1    \\ %\midrule
% Kinetics Fine-tune & 10.6 & 1.26 & 75.9 & 46.7    \\
% From scratch & 12.7                   & 1.45                    & 69.6 & 40.7    \\
% \midrule
% Kinetics Linear & 12.9                   &  1.53                    & 69.2 &  37.8   \\
% FPS Linear     & 14.0                 &     1.65               & 65.3 &   36.6  \\
% CTC Linear             & 18.0        & 1.95          &  52.0    & 25.3        \\
% Sorting Linear \cite{xu2019self}              &  20.9       &   2.20        & 43.3     &    18.3     \\
% Scratch Linear  &  19.3                & 2.03                  & 47.8 &  21.6   \\ \midrule
% %Future prediction       & 18.9        & 2.04          & 47.2     &  21.7       \\
% Motion Magnitude              &  18.6       &   2.06        &  50.7    & 23.1        \\
% Actions withheld              & 12.9        & 1.52          & 68.7     & 39.6        \\ 
% Random withheld              &  12.2       &  1.40         &  69.7    &  39.5       \\\midrule
% Middle Prior      & 14.9                  & 1.63                    & 53.1 & 21.0    \\
% Chance  & 30.7                  & 3.11                  & 25.9   & 6.8    \\ \bottomrule
% \end{tabular}
\begin{tabular}{l | c c}
\toprule
                & \multicolumn{2}{c}{\textbf{Accuracy within}} \\
                %\cmidrule{2-3}
\textbf{Method} & \textbf{1 sec} & \textbf{0.25 sec} \\ \midrule
Human Consistency   & 88.0   & 62.1    \\ %\midrule
Kinetics Supervision (Fine-tune) & 75.9 & 46.7    \\
%From scratch & 12.7                   & 1.45                    & 69.6 & 40.7    \\
Kinetics Supervision (Linear)  & 69.2 &  37.8   \\ \midrule
Video Speed (ours) & \textbf{65.3} &  \textbf{36.6}  \\
Video Context \cite{oord2018representation}  &  52.0    & 25.3        \\
Video Sorting \cite{xu2019self}  & 43.3     &    18.3     \\  \midrule
Scratch  & 47.8 &  21.6   \\
%Future prediction       & 18.9        & 2.04          & 47.2     &  21.7       \\
Motion Magnitude    &  50.7    & 23.1        \\
%Actions withheld              & 12.9        & 1.52          & 68.7     & 39.6        \\ 
%Random withheld              &  12.2       &  1.40         &  69.7    &  39.5       \\\midrule
Middle Prior       & 53.1 & 21.0    \\
Chance        & 25.9   & 6.8    \\ \bottomrule
\end{tabular}
%}
\vspace{-1em}
\caption{\textbf{Temporal Localization:} We evaluate the model at localizing the onset of unintentional action for two different temporal thresholds of correctness. Although there is high human agreement on this task, there is still a large gap for both supervised and self-supervised models.}
\label{tab:loc}
% \end{table}
\vspace{1em}
% \begin{table}[tb]
% \resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{@{}l|c}
\toprule
\textbf{Method}           &  \textbf{Accuracy}  \\ \midrule
Kinetics Supervision & 59.7             \\ \midrule
Video Speed (ours)                      & \textbf{56.7}            \\
Video Context \cite{oord2018representation}                     & 51.2                \\
Video Sorting   \cite{xu2019self}           & 51.0            \\  \midrule
Scratch                        & 50.8  \\
Chance                 & 50.0        \\ \bottomrule
\end{tabular}
\vspace{-1em}
\caption{\textbf{Anticipation:} We evaluate performance at predicting the onset of failure before it happens (1.5 seconds into future) by fine-tuning our models. The best performing self-supervised visual clue we considered is video speed.\vspace{-2em}}
\label{tab:ant}
\end{table}

\subsection{Anticipation}\label{sec:exp_ant}

We also evaluate the representation at anticipating the onset of unintentional action. To do this, we train the models with self-supervision as before, but then fine-tune them for a three-way classification task to predict the labels $1.5$ seconds into the future.  Table \ref{tab:ant} reports classification accuracy for the prediction. Features from the the video speed prediction model obtain the best self-supervised performance. However, the model with full Kinetics supervision obtains about 3\% higher performance, suggesting there is still room for self-supervised learning to improve on this task. 

% In addition to failure classification and localization, an interesting task that emerges from this dataset is the anticipation of yet-to-occur failures. This is a particularly challenging task; in some cases, it is very difficult --- such as someone walking down the street and suddenly tripping --- though in others it may be easier, such as someone learning to ride a bike and swaying from side to side, unbalanced. To train models, we set $y(x_t) = y_{t+k}$ instead of $y_t$, \ie we shift labels over by $k$ seconds (we use $k=1.5$ to avoid overlap, since video context is 1 second long).\par
% To evaluate the model, we use a slightly different metric than in \ref{sec:exp_clsloc}, since we are not interested in the trivial task of anticipating the label ``after failure" (once you are after a failure, it is easy to predict that you will continue to be). Therefore, we compute accuracy only for two way classification, where $y_{t+k} \in \{0,1\}$.\par
% While a model trained from scratch barely exceeds chance, a strong initial representation leads to significant gains in performance. Anticipating unintentional action before its onset remains a particularly challenging task.


% \begin{table}[tb]
% \resizebox{\columnwidth}{!}{
% \begin{center}
% \begin{tabular}{@{}l|llll@{}}
% \toprule
% \textbf{Initialization}           &  \textbf{Error (\%)} & \textbf{Error (sec)}& \textbf{Acc@1s} & \textbf{Acc@0.25s} \\ \midrule
% Kinetics                 & 16.0 & 1.78 & 59.0 & 23.1               \\
% FPS                       & 16.2 & 1.76 & 56.5 & 18.9             \\
% CTC                      &          &&  &        \\
% Sorting   \cite{xu2019self}           &  &&   &             \\
% From scratch                        & 17.1 & 1.87 & 53.7 & 18.3     \\ \midrule
% Chance                 & 30.7                  & 3.11       & 25.9                         & 6.8             \\ \bottomrule
% \end{tabular}
% \end{center}
% }
% \caption{\textbf{Failure anticipation:} TODO \de{find a better metric}.}
% \label{tab:ant}
% \end{table}
% \begin{table}[tb]
% % \resizebox{\columnwidth}{!}{
% \begin{center}
% \begin{tabular}{@{}l|ll@{}}
% \toprule
% \textbf{Initialization}           &  \textbf{Area Under Curve} & \textbf{F1 Score}\\ \midrule
% Kinetics                 & 59.3 & 38.9             \\
% FPS                       & 56.9 & 39.8             \\
% CTC                      &          &       \\
% Sorting   \cite{xu2019self}           &  &             \\
% From scratch                        & 55.5 & 38.4      \\ \midrule
% Chance                 &                  &                     \\ \bottomrule
% \end{tabular}
% \end{center}
% % }
% \caption{\textbf{Failure anticipation:} TODO \de{decide on metric}.}
% \label{tab:ant}
% \end{table}


\subsection{Analysis}\label{sec:exp_analysis}


%\textbf{Motion magnitude:} One potentially undesirable signal that could be used to solve failure prediction tasks is low-level motion, since failures are sometimes characterized by sharp, unexpected movements and videos are often filmed by handheld shaky cameras whose operators might react to the failure with rapid movement. We show that considering low-level motion cues alone does not allow for success at our tasks by training a model on the three-way classification task just as in Section \ref{sec:learning_sup}, but replacing the RGB video input with a fixed-bin histogram of its flow magnitudes. We show in Tables \ref{tab:loc} and \ref{tab:cls} that this method, while better than chance at most metrics, does not approach the performance of the proposed methods. Accordingly, visualizing flow histograms before, at, and after failure reveals that they do not exhibit any meaningful qualitative properties. \par

Our results so far have suggested that there are perceptual clues in unlabeled video that we can leverage to learn to recognize intentionality. In this subsection, we break down performance to analyze strengths and limitations.

\begin{figure}[tb]
\centering
    %\resizebox{\columnwidth}{!}{
      \begin{tabular}{crP{1.25cm}P{1.25cm}P{1.25cm}}
%\toprule
 && \multicolumn{3}{c}{\textbf{Predicted Label}} \\ %\cmidrule(l){2-4} 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{True Label}}}&& {Intent.}    & {Failure} & {Unintent.} \\ %\cmidrule(l){2-4} 
 & {Intention}        & \cellcolor{afterfail!62}62.2              & \cellcolor{afterfail!10}10.2       & \cellcolor{afterfail!28}27.6          \\
&{Failure}          & \cellcolor{afterfail!23}22.9              & \cellcolor{afterfail!44}43.9       & \cellcolor{afterfail!33}33.2          \\
&{Unintentional}         & \cellcolor{afterfail!23}23.3              & \cellcolor{afterfail!9}9.3        & \cellcolor{afterfail!67}67.4 \\
& & \multicolumn{3}{c}{(a) Kinetics + Fine-tune} 
\end{tabular}
%}\resizebox{\columnwidth}{!}{
\\
\vspace{1em}
      \begin{tabular}{crP{1.25cm}P{1.25cm}P{1.25cm}}
%\toprule
% && \multicolumn{3}{c}{\textbf{Predicted Label}} \\ %\cmidrule(l){2-4} 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{True Label}}}&& {Intent.}    & {Failure} & {Unintent.} \\ %\cmidrule(l){2-4} 
 & {Intentional}        & \cellcolor{afterfail!43}43.0 & \cellcolor{afterfail!19.5}19.5 & \cellcolor{afterfail!37}37.4 \\
&{Failure}          & \cellcolor{afterfail!24}24.8 & \cellcolor{afterfail!43}43.5 & \cellcolor{afterfail!31}31.5 \\
&{Unintentional}         & \cellcolor{afterfail!21}21.5 & \cellcolor{afterfail!16}16.0 & \cellcolor{afterfail!62}62.5 \\
& & \multicolumn{3}{c}{(b) Video Speed + Linear} 
\end{tabular}
%}
\vspace{-1em}
\caption{\textbf{Classification Confusion Matrices:} We compare the confusion matrices for (\textbf{a}) Kinetics supervision and (\textbf{b}) self-supervision. One key difference is the self-supervised model often confuses intentional action with the start of failure, suggesting there is substantial room for improving fine-grained localization of intentionality.}
    \label{tbl:conf}
\end{figure}

\textbf{Frequent Confusions:} Figure \ref{tbl:conf} compares the confusion matrices for both the video speed representation and Kinetics supervised representation. In both cases, the most challenging point to predict is the boundary between intentional and unintentional action, which we label the ``Failure'' point. Moreover, a key difference between models is that the self-supervised model more often confuses intentional action with the start of failure. Since the supervised model performs better here, this suggests there is still substantial room to improve self-supervised models at fine-grained localization of intentionality. 

\textbf{Visualization of Learned Features:} To qualitatively analyze the learned feature space, Figure \ref{fig:nn} visualizes nearest neighbors between videos using the representation learned by predicting the video speed, which is the best performing self-supervised model. We use one video clip as a query, compute features from the last convolutional layer, and calculate the nearest neighbors using cosine similarity over a large set of videos not seen during training. Although this feature space is learned without ground-truth labels, the nearest neighbors are often similar activities and objects, suggesting that learning to predict the video speed is promising incidental supervision for learning features of activity.


\textbf{Performance Breakdown:}
We manually labeled a diagnostic set of 270 videos into nine types that characterize the cause of unintentional action.
Figure \ref{fig:breakdown} reports performance of models broken down by video type. The most challenging cases for our models are when the unintentional action is caused by environmental factors (such as slipping on ice) or unexpected interventions (such as a bird swooping in suddenly). Moreover, performance is comparatively low when the person in the video has limited visibility, such as due to occlusions, which motivates further work in gaze estimation \cite{recasens2015they,kellnhofer2019gaze360}, especially in video. Another challenge is due to limited knowledge, such as understanding that fire is hot. In contrast, the model has better performance at recognizing unintentional action in multi-agent scenes, likely because multi-agent interaction is more visually apparent. 

%The most challenging videos for humans tend to be unintentional action arising from poor planning. In these cases, the inevitability of failure often becomes clear at an early point, and annotators exhibit higher variance in their localization.

% \textbf{Action Memorization:} We also analyzed how the model generalizes to action categories not seen during training. We first removed 25\% of the training videos at random, trained the full model, and computed classification performance. 

% We removed 25\% of the training data

% One possible way for our models to solve the tasks in the dataset, which would circumvent the need to learn about intention, is to memorize the ``prototypical appearance" of all actions, and simply flag clips that significantly deviate from the prototype of the recognized action. To demonstrate that the model does not do this, we ablate 25\% of the training data in two ways: first, we remove random videos; second, we remove videos predicted as belonging to semantically-related Kinetics classes (specifically, athletics and sports videos).\par
% We then train models from scratch on both reduced datasets. We show that for all metrics, the model with actions withheld does not perform significantly worse (1\% worse on localization accuracy) than the model with random videos withheld, despite the frequency of the removed actions in the test set. This suggests that our models are able to learn about the intrinsic nature of failure and unintentional action, as opposed to learning a notion of what an action should look like.



\begin{figure}[t]
\includegraphics[width=\columnwidth]{figs/oops_nn.pdf}
\caption{\textbf{Nearest Neighbors on Self-supervised Features:} We visualize some of the nearest neighbors from the feature spaced learned by predicting video frame rate. The nearest neighbors tend to be similar activities despite significant variation in appearance.\vspace{-1em}}
\label{fig:nn} 
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/category_err.pdf}
\vspace{-2em}
\caption{\textbf{Performance Breakdown:} We annotate a diagnostic set of videos into different categories of unintentional action in order to break down model performance and limitations. See text for discussion.\vspace{-1em}}
\label{fig:breakdown} 
\end{figure}




% \de{here} As shown in Figure \ref{fig:breakdown}, for ``unexpected" category, the performance of the proposed models has the largest gap with humans. This suggests that this type of failures is more unpredictable for the proposed models. This motivates further work on models of uncertainty \bc{cite}. We also note that humans tend to make much higher error on ``planning error" type of failures. We hypothesis that ``planning error" has more complex structure which maybe hard for humans to agree. The performance gaps between supervised and self-supervised feature learning implies future potentials on improving the learning algorithms.



% % to supplementary
% \begin{table}[h]
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}l|llll@{}}
% \toprule
% \textbf{Failure type}           &  \textbf{Cause of failure}  \\ \midrule
% Limited skill                 & Inadequate expertise at the attempted task,\\ \eg an amateur biking down a steep hill            \\ \midrule
% Limited knowledge                       &  Lack of common-sense knowledge,\\ \eg a child touching a fire \\ \midrule
% Environmental                      & Interference by environmental factors,\\ \eg slippery road due to rain  \\ \midrule
% Unexpected           & Unpredictable interruption or behavior by third party,\\ \eg car driving into backyard    \\ \midrule
% Limited visibility      & \de{here}  \\ \midrule
% Planning error      & Bad initial plans or pranks  \\ \midrule
% Execution error      & Correct intention but flaw carrying out  \\ \midrule
% Single-agent         & Involvement of a single person        \\ \midrule
% Multi-agent         & Multi-agent interaction        \\ \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{\textbf{Types of failures:} to study model performance on different types of failures, we annotate a subset of test set video clips and sort them into nine sub-categories of failures. We briefly describe each category above; model performance is broken down accordingly in Figure \ref{fig:breakdown}.}
% \label{tab:category}
% \end{table}




==> intro.tex <==
\section{Introduction}\label{sec:intro}

From just a glance at a video, we can often tell whether a person's action is intentional or not. For example, Figure \ref{fig:teaser} shows a person attempting to jump off a raft, but unintentionally tripping into the sea. In a classic series of papers, developmental psychologist Amanda Woodward demonstrated that this ability to recognize the purposefulness behind action is learned by children during their first year \cite{woodward1999infants,woodward2009infants,brandone2009you}. However, predicting the purpose of action has remained elusive for machine vision. 
Recent advances in action recognition have largely focused on predicting the physical motions and atomic actions in video \cite{kay2017kinetics,gu2018ava,monfort2019moments}, which captures the means of action but not the goal of action. 

\enlargethispage{-6.6cm} % FOR HACK

We believe a key limitation for perceiving visual intentionality has been the lack of realistic data with natural variations of intention. Although there are now extensive video datasets for action recognition \cite{kay2017kinetics,gu2018ava,monfort2019moments}, people are usually competent, which causes datasets to be biased towards successful outcomes. However, this bias for success makes discriminating and grounding visual intentionality difficult for both learning and quantitative evaluation. 

\begin{figure*}[t]
\includegraphics[width=\linewidth]{figs/datasetbignewspacing.png}
\caption{\textbf{Examples of intentional and unintentional action in the \oops dataset:}
For each pair of frames, we show intentional and unintentional action from our dataset. By crawling publicly available ``fail'' videos from the web, we can create a diverse and in-the-wild dataset of unintentional action.}
\label{fig:dataset} 
\end{figure*}

\bc{modified starting here ...}
We introduce a new annotated dataset of intentional and unintentional action, which we have collected by crawling publicly available ``fail'' videos from the web. Figure \ref{fig:dataset} shows some examples. Due to the popularity of these videos, we believe this is a promising resource to collect a large number of videos that show a balance of purposeful and non-purposeful action across unconstrained, in-the-wild situations. Our video dataset, which we will publicly release, is both large (over 50 hours of video) and diverse (covering hundreds of scenes and activities). We annotated videos with temporal location at which the failure happens. This is because a failure generally represents a transition from intentional to unintentional action, which makes failure a good signal to look at for studying intentionality. We propose three tasks on this dataset: classifying the purposefulness of action, localizing the transition from intentional to unintentional, and forecasting the onset of unintentional action in the future.


% We annotated videos with the temporal location at which the video transitions from intentional to unintentional action. We propose three tasks on this dataset: classifying the purposefulness of action, localizing the transition from intentional to unintentional, and forecasting the onset of unintentional action in the future. 

Along these tasks, we target at a fundamental property of video: \emph{what intrinsic visual clues are available to detect intentional action?} As we show in our experiment, human labeled data can provide clear signals to supervise the learning process. However, simply relying on supervision signals will not be ideal since intentionality is a relative subjective signal and it is often expensive and impractical to gather human labels.

In this paper, we use unlabeled and raw videos, and the natural speed of events as a self-supervised learning signal to learn a representation of intentionality. Inspired by studies in psychology and cognitive science \cite{caruso2016slow} that human's judgement of intent can be manipulated by changing the replay speed of videos, we propose to use duration detection as a pretext task to encourage the models to learn useful representations for intentionality prediction.

We extensively study the performance of our proposed method by comparing it with multiple baseline methods. Experiments and visualizations suggest that our duration prediction method learns effective feature representations that can be fine-tuned for various intentionality prediction tasks including classification, localization and anticipation. Our model outperforms multiple state-of-the-art self-supervised methods and features trained from scratch. Though without any given labels, the model performs substantially close to features trained from supervised action classification tasks. Moreover, through systematic ablation studies, we show that our model does not simply utilize low-level bias in the dataset such as motion magnitude and action categories.
% Since young children recognize intentionality, this is a perception task 

The two primary contributions of this paper are a new dataset for visual intentionality and a self-supervised representation for predicting intentionality. The remainder of this paper will describe these contributions in detail. In Section \ref{sec:related}, we first review related work in action recognition and visual self-supervised learning. In Section \ref{sec:dataset}, we introduce our dataset and analyze it. In Section \ref{sec:learning}, we propose a self-supervised learning approach to learn visual representations of intentionality along with other self-supervised baselines. In Section \ref{sec:exp}, we present both quantitative and qualitative experiments to analyze our model. Due to the importance of this problem, we will release all data, software, and models.




% ---




% From just a glance at a video, we can quickly determine whether a person's action is intentional or accidental. Although the video in \figref{fig:teaser} shows an activity you may have never seen before, you can easily predict the person's goals and know whether they intended to perform this action. In fact, at a very young age, children are able to understand the intention behind other people's behavior \cite{woodward2009infants, brandone2009you}. Despite the ease of this task to humans, computer vision systems are yet to be able to infer intention and goals. \par



% Though recently, much progress has been made in advancing action recognition systems, these systems do not distinguish between successful (intentional) and failed (accidental) actions. In this paper, we approach learning intention from the perspective of learning to predict unintentional actions, or failure moments, in video. The presence of a failure provides counterfactual evidence toward the actor's intended action, and thus is a natural signal toward learning a richer representation of human behavior.\par
% We introduce a set of {\em failure prediction tasks}, accompanied by a large-scale dataset of diverse real-world fail videos, to learn to detect and localize human failure in video. Such an ability is a key element of successfully modeling human behaviors from visual observations, and we believe \de{here - talk about self supervised depending on results}


